Common envelopes in massive stars: Towards the role of radiation pressure and recombination energy in ejecting red supergiant envelopes

We perform 3D hydrodynamical simulations of a common-envelope event involving a 12 solar mass red supergiant donor. Massive stars are expected to be qualitatively different from low-mass stars as their envelopes have significant support from radiation pressure, which increases both the final separation and amount of mass ejected through the common-envelope interaction. We perform adiabatic simulations that include radiation energy through the equation of state, which results in ejecting 60 per cent more mass (up to two thirds of the total envelope mass becoming unbound, or more) and yield a 10 per cent larger final separation compared to simulations that assume an ideal gas. When also including recombination energy, we find that at least three quarters of the envelope, and possibly the entire envelope, may be unbound. The final separation further increases by almost 20 per cent. The additional amount of ejected material is mainly due to energy injected from helium recombination. Hydrogen recombination plays a comparatively small role, as it mainly occurs in gas that has already become unbound. We conclude that the internal energy of the envelope can be a significant energy source for ejecting the common envelope, but ultimately radiation transport and convection need to be included.

==> app/final_sep.tex <==
\subsection{Fitting the final separation}
\label{app:final_sep}

\begin{figure*}
	\centering
	\includegraphics[width=\linewidth]{figs/fit_final_sep.eps}
	\caption{Linear least squares fits (black dashed line) to $\ln(-\dot{a}(t))$ (blue line) past the dynamical inspiral for the $q = 0.25$ simulations, showing from left to right results for the ideal gas, gas + radiation, and full equation of state. This is equivalent to an exponential fit to the $a(t)$. The fitting coefficients, defined in equation (\ref{eq:final_sep}), are labelled in each panel. In particular, $a_f$ gives the final separation of each simulation.}
	\label{fig:fit_final_sep}
\end{figure*}

A key goal of \ac{CE} simulations is to determine the final separation of the binary orbit. However, the orbital separation does not stall completely after the plunge-in, transitioning to a slow spiral-in at a rate of several solar radii per year. We extract the final separation by fitting the semi-major axis during the slow spiral-in with an exponential function (equation (\ref{eq:final_sep})). We first solve for the semimajor axis, $a(t)$, of the stellar cores given their masses and instantaneous positions and velocities, then perform a least squares fit to equation (\ref{eq:final_sep}).

In Figure \ref{fig:fit_final_sep}, we plot $\ln(-\dot{a}(t))$ for the $q=0.25$ simulations, confirming that it is approximately linear, as expected if the semi-major axis were reasonably well modelled by a decaying exponential function by. The noise in the $\ln(-\dot{a}(t))$ curves (blue) is associated with numerical differentiation. The fitting parameters in equation (\ref{eq:final_sep}) are displayed in each panel, including the final separation, $a_f$.

==> app/resolution.tex <==
\section{Resolution study}
\label{app:resolution}




==> discussion/drag.tex <==
\subsection{Inspiral dynamics and gravitational drag} \label{subsec:drag}
\begin{itemize}
	\item Comparing simulation plunge-in and wind tunnel prediction
	\item A plot comparing separation vs. time curve for analytical model and for actual simulation, for MESA, gas+rad, and ideal EoSs, and for fixed drag coefficients and interpolated drag coefficients
	\item Version of the above but showing the 2-d inspiral
\end{itemize}

==> discussion/nebula.tex <==
\subsection{Nebula formation}
\label{subsec:nebula}
\begin{figure*}
	\centering
	\includegraphics[width=\linewidth]{figs/nebula.png}
	\caption{\ilya{Here and elsewhere -- clearly list EOS, $q$ and resolution for every plot.  $10^5 Rsol$ scale legend is very small (also, use $R_\odot$).} Sequence of surface renderings showing the expansion of the nebula formed from the common-envelope. The gas that is expelled during the dynamical inspiral forms a torus aligned with the orbital plane \ilya{What is the plane of the plots?}, while bipolar lobes are launched towards the end of the dynamical inspiral along the axis perpendicular to the orbital plane. \mike{To-do: Adjust dimensions of plot, combine with radial velocity plot. Put colorbar underneath. Plot for 500k particles?}\miguel{Maybe use Mach instead of radial velocity for this render plots.} }
	\label{fig:nebula}
\end{figure*}

\begin{figure*}
	\centering
	\includegraphics[width=\linewidth]{figs/vr_vs_r.eps}
	\caption{Plots of radial velocity, $v_r$, against radius, $r$ of \ac{SPH} particles for three different snapshots at late stages of the common-envelope phase after the dynamical inspiral, corresponding to the same snapshots in Fig. \ref{fig:nebula}. The plot colour indicates the particle density \ilya{Include colorbar, or say that red is high and blue is low density?}. Some of the outwardly-expanding \ac{SPH} particles fall along two straight lines, demonstrating homologous expansion of the post-common-envelope nebula. The long-dashed and short-dashed lines indicate the expected $v_r$-$r$ relation for a homologously expanding outflow launched at 34.1 and 29.7 yr, which correspond to the bipolar lobes and the torus, respectively, as seen in Fig. \ref{fig:nebula}. The maximum velocity of these lines is roughly the escape velocity at the surface of the donor star.  \ilya{Explicitly discuss velocity or kinetic energy of fast ejecta in the text -- looks like at least some material is given too much KE by a factor of a few?} \mike{To-do: Adjust dimensions of plot, combine with surface rendering.}
	% Equation for lobe: f(x,t) = 6.96e10/(t-29.7)/3.15e7/1e5 *x = 0.022/(t-29.7)*x
	% Equation for torus: f(x,t) = 0.022/(t-34.1)*x
	}
	\label{fig:vr_vs_r}
\end{figure*}
